Web Retrieval Agents for Evidence-Based Misinformation Detection

This paper develops an agent-based automated fact-checking approach for detecting misinformation. We demonstrate that combining a powerful LLM agent, which does not have access to the internet for searches, with an online web search agent yields better results than when each tool is used independently. Our approach is robust across multiple models, outperforming alternatives and increasing the macro F1 of misinformation detection by as much as 20 percent compared to LLMs without search. We also conduct extensive analyses on the sources our system leverages and their biases, decisions in the construction of the system like the search tool and the knowledge base, the type of evidence needed and its impact on the results, and other parts of the overall process. By combining strong performance with in-depth understanding, we hope to provide building blocks for future search-enabled misinformation mitigation systems.

==> jacob_discussions.tex <==
% \section{Discussion and Future Works}

Pairing the ``Chat with RAG'' model from Cohere with a more powerful main agent enabled us to exceed the performance of both Chat with RAG and the main LLM agent itself. We hypothesize that compared to \texttt{mixtral-instruct-8x7B-v0.1} or the model behind Cohere's Chat with RAG (Command R, in our experiments), the OpenAI LLMs are capable of doing a better job at decomposing the statement. By asking better questions, the models retrieved information that was more relevant and achieved better overall performance. In future work, we plan to test the effect of decomposition and query generation versus final evaluation by taking the decomposition and search results of GPT-4 and making a final prediction with weaker models.

We observe that the capability of the generator model might create a bottleneck for the overall performance of the pipeline. For instance, while both \texttt{gpt-3.5-turbo} and \texttt{gpt-4-0613} had the same knowledge cutoff, \texttt{gpt-4-0613} demonstrated a significantly better performance gain. A preliminary review of the model generations suggested that queries from \texttt{gpt-4-0613} were more concise, allowing it to retrieve more relevant results from web searches. While additional analyses are required, we note that the quality of the generated search queries might be the reason why adding search to \texttt{vicuna-13b-v1.5} did not improve overall performance by much.

Additionally, we note that the performance gain from search is more pronounced with \texttt{gpt-4-turbo-0125} ($+12.8\%$ F1, 2023/12 cutoff) as the generator model than with \texttt{gpt-3.5-turbo} ($+5.4\%$ F1, 2021/03 cutoff). We find this result surprising, especially given that when compared with \texttt{gpt-3.5-turbo}, \texttt{gpt-4-turbo-0125} has a more recent knowledge cutoff. Specifically, the LIAR-New dataset includes only statements from fact-checking articles from October 2021 and later, meaning the world knowledge of \texttt{gpt-4-turbo-0125} (up to 2023/12) encompasses the dataset's entire time span, while that of \texttt{gpt-3.5-turbo} (up to 2021/03) includes none of it. Our initial hypothesis was that this model would benefit less from web search, but that was not the case. We suspect that this unexpected trend might be related to the relative differences between the logic capabilities of these two LLMs, as well as the limited capacity of the models to memorize facts. However, additional work will be required to fully understand this difference.

%We also see a decrease in performance from using search when statements contain an unspecified speaker and location. We hypothesize that speaker and location information is more difficult to retrieve without direct specification, because they create a variety of scenarios the statement may refer to.  We reason that if we can identify the category of missing information in a statement, we can selectively invoke web retrieval if we can expect it to be effective. With selective web retrieval, we can both improve the overall performance, and reduce computational costs.


